Torsion contact forms in three dimensions have two or infinitely many Reeb orbits

We prove that every nondegenerate contact form on a closed connected three-manifold, such that the associated contact structure has torsion first Chern class, has either two or infinitely many simple Reeb orbits. By previous results it follows that under the above assumptions, there are infinitely many simple Reeb orbits if the three-manifold is not the three-sphere or a lens space. We also show that for non-torsion contact structures, every nondegenerate contact form has at least four simple Reeb orbits.

==> infinity-foliation.tex <==
\section{From a special curve to a foliation}

The goal of this section is to prove Proposition~\ref{prop:foliation} below. As we will see, this proposition implies that a special curve gives rise to a foliation of a subset of $Y$.

 Following Wendl \cite{wendl-jems}, define the {\bf normal Chern number\/} of $u$ by
\[
c_N(u) = \frac{1}{2}\left(2g(u) - 2 + \op{ind}(u) + h_+(u)\right).
\]
Let $\M^J_u$ denote the component of the moduli space of $J$-holomorphic curves in $\mathbb{R} \times Y$ that contains $u$.  

\begin{proposition}
\label{prop:foliation}
Let $(Y,\lambda)$ be a nondegenerate contact three-manifold, and let $J$ be a $\lambda$-compatible almost complex structure\footnote{In Proposition~\ref{prop:foliation} it is not necessary to assume that $J$ is generic.} on $\R\times Y$. Let $C$ be a nontrivial irreducible embedded $J$-holomorphic curve in $\R\times Y$ such that:
\begin{description}
\item{(i)} Every $C'\in\M^J_C$ is embedded in $\R\times Y$.
\item{(ii)} $c_N(C)=0$.
\item{(iii)} $C$ does not have two positive ends, or two negative ends, at covers of the same simple Reeb orbit.
\item{(iv)} Let $\gamma$ be a simple Reeb orbit with rotation number $\theta\in\R/\Z$. If $C$ has a positive end at an $m$-fold cover of $\gamma$, then $\op{gcd}(m,\floor{m\theta})=1$. If $C$ has a negative end at an $m$-fold cover of $\gamma$, then $\op{gcd}(m,\ceil{m\theta})=1$.
\end{description}
Then:
\begin{description}
\item{(a)} For every $C'\in\M^J_C$, the projection of $C'$ to $Y$ is an embedding.
\item{(b)} If $g(C)=h_+(C)=0$, then the projections of the curves $C'\in\M^J_C$ to $Y$ give a foliation of an open subset of $Y$.
\end{description}
\end{proposition}

This proposition is a slight generalization of \cite[Prop.\ 3.4]{wh}, and the ideas in the proof go back to \cite{hwz-emb}.

We first need to recall the significance of the normal first Chern number. Let $u$ be an immersed $J$-holomorphic curve in $\R\times Y$ with domain $\Sigma$, and let $N\to\Sigma$ denote the normal bundle to $u$. Then $u$ has a well-defined deformation operator
\[
D_u: L^2_1(\Sigma,N) \longrightarrow L^2(\Sigma,T^{0,1}\Sigma\tensor N),
\]
see e.g. \cite[\S2.3]{bn}. The derivative at $u$ of a one-parameter family of curves in $\M^J_u$ defines an element of $\Ker(D_u)$.

If $\psi\in\Ker(D_u)$ does not vanish identically (and $u$ is irreducible), then $\psi$ has only finitely many zeroes, all of which have positive multiplicity; see the review in \cite[Prop.\ 3.4]{wh}. We can then define winding numbers of $\psi$ around the ends of $u$ as follows. Suppose that $u$ has positive ends at $m_i$-fold covers of simple Reeb orbits $\alpha_i$, and negative ends at $n_j$-fold covers of simple Reeb orbits $\beta_j$. Let $\tau$ be a trivialization of $\xi$ over the Reeb orbits $\alpha_i$ and $\beta_j$. Let $\op{wind}_{i,\tau}^+(\psi)$ denote the winding number of $\psi$ around the positive end of $u$ at $\alpha_i^{m_i}$, as measured using the trivialization $\tau$. Likewise, let $\op{wind}_{j,\tau}^-(\psi)$ denote the winding number of $\psi$ around the negative end of $u$ at $\beta_j^{n_j}$ with respect to $\tau$.

It was shown in \cite{hwz-emb}, see the review in \cite[\S5.1]{bn}, that the above winding numbers are bounded by
\begin{equation}
\label{eqn:windCZ}
\begin{split}
\op{wind}_{i,\tau}^+(\psi) &\le \floor{\CZ_\tau\left(\alpha_i^{m_i}\right)/2}\\
\op{wind}_{j,\tau}^-(\psi) &\ge \ceil{\CZ_\tau \left(\beta_j^{n_j}\right)/2}.
\end{split}
\end{equation}
If $\theta_{i,\tau}^+$ denotes the rotation number of $\alpha_i$ with respect to $\tau$, and if $\theta_{j,\tau}^-$ denotes the rotation number of $\beta_j$ with respect to $\tau$, then we can rewrite the above inequalities as
\begin{equation}
\label{eqn:windtheta}
\begin{split}
\op{wind}_{i,\tau}^+(\psi) &\le \floor{m_i\theta_{i,\tau}^+}\\
\op{wind}_{j,\tau}^-(\psi) &\ge \ceil{n_j\theta_{j,\tau}^-}.
\end{split}
\end{equation}

\begin{lemma}
\label{lem:normalcn}
Let $(Y,\lambda)$ be a nondegenerate contact 3-manifold and let $J$ be a $\lambda$-compatible almost complex structure on $\R\times Y$. Let $u$ be an immersed irreducible $J$-holomorphic curve in $\R\times Y$. Suppose that $c_N(u)=0$. Let $\psi$ be a nonzero element of $\Ker(D_u)$. Then:
\begin{description}
\item{(a)}
$\psi$ is nonvanishing.
\item{(b)}
Equality holds in the inequalities \eqref{eqn:windCZ}.
\end{description}
\end{lemma}

\begin{proof}
Let $\tau$ be a trivialization of $\xi$ over the Reeb orbits at whose covers $u$ has ends. The algebraic count of zeroes of $\psi$ is then given by
\begin{equation}
\label{eqn:psi0}
\#\psi^{-1}(0) = c_1(N,\tau) + \op{wind}_{\tau}(\psi)
\end{equation}
where
\begin{equation}
\label{eqn:windtaudef}
\op{wind}_\tau(\psi) = \sum_{i}\op{wind}_{i,\tau}^+(\psi) - \sum_{j}\op{wind}_{j,\tau}^-(\psi).
\end{equation}
As in \cite[Lem.\ 3.1(a)]{pfh2}, we have
\begin{equation}
\label{eqn:oldadj}
c_1(N,\tau) = c_\tau(u) - \chi(\Sigma)
\end{equation}
where $\Sigma$ denotes the domain of $u$.
By \eqref{eqn:windCZ} and \eqref{eqn:windtaudef}, since $\op{CZ}_\tau(\gamma)$ is even if and only if $\gamma$ is positive hyperbolic, we have
\begin{equation}
\label{eqn:2wind}
2\op{wind}_\tau(\psi) \le  \CZ_\tau^{\op{ind}}(u) - p(u) + h_+(u),
\end{equation}
where $p(u)$ denotes the total number of ends of $u$.

Combining \eqref{eqn:psi0}, \eqref{eqn:oldadj}, and \eqref{eqn:2wind}, we obtain
\begin{equation} \label{eqn:zeronchn}
\begin{split}
2\#\psi^{-1}(0) &\le 2c_\tau(u) - 2\chi(\Sigma) + \CZ_\tau^{\op{ind}}(u) - p(u) + h_+(u)\\
&= \op{ind}(u) - \chi(\Sigma) - p(u) + h_+(u)\\
&= 2c_N(u).
\end{split}
\end{equation}

Since $c_N(u)=0$ and all zeroes of $\psi$ have positive multiplicity, we have that $\#\psi^{-1}(0)=0$, establishing (a). To deduce (b), note that the inequality \eqref{eqn:zeronchn} is in fact an equality. This implies that equality also holds in \eqref{eqn:2wind} and hence \eqref{eqn:windCZ}.
\end{proof}

\begin{lemma}
\label{lem:embedding}
Under the hypotheses in Proposition~\ref{prop:foliation}, if $C'\in\M^J_C$, then:
\begin{description}
\item{(a)}
The projection of $C'$ to $Y$ is an embedding.
\item{(b)}
If $C'$ is not obtained from $C$ by translation of the $\R$ factor in $\R\times Y$, then the projections of $C$ and $C'$ to $Y$ are disjoint.
\end{description}
\end{lemma}

\begin{proof}
We proceed in four steps. We continue to use the notation from \eqref{eqn:windCZ} and \eqref{eqn:windtheta}.

{\em Step 1.\/} We first show that the projection of $C'$ to $Y$ is an immersion.

For any $C'\in\M^J_C$, the projection of $\partial_s$ (the derivative of the $\R$ coordinate on $\R\times Y$) to the normal bundle $N$ of $C'$ is a nonzero element of $\Ker(D_{C'})$, since it is the derivative of the family of curves obtained by translating $C'$ in the $\R$ direction. Since we are assuming that $C'$ is not a trivial cylinder, the projection of $\partial_s$ to $N$ does not vanish identically. We have that $c_N(C')=0$ and by hypothesis (i), we have that $C'$ is embedded. Thus, we may apply Lemma~\ref{lem:normalcn}(a) to conclude that the projection of $\partial_s$ to $N$ is nonvanishing. This means that the projection of $C'$ to $Y$ is an immersion. 

{\em Step 2.\/} We next show that if $C'\in\M^J_C$ and $C\neq C'$, then the algebraic count of intersections of $C$ and $C'$ in $\R\times Y$ does not depend on $C'$.

It follows from the definition of $Q_\tau$ in \cite[\S2.7]{ir} that the algebraic count of intersections of $C$ and $C'$ is given by
\[
\#(C\cap C') = Q_\tau(C) + \ell_\tau(C,C'),
\]
where $\ell_\tau(C,C')$ is the ``asymptotic linking number'' of $C$ and $C'$ with respect to $\tau$, defined in \cite[\S2.7]{ir}.

To analyze this asymptotic linking number, let $\op{wind}_{i,\tau}^+(C)$ denote the winding number of $\partial_s$ around the positive end at $\alpha_i^{m_i}$ with respect to $\tau$. Define $\op{wind}_{j,\tau}^-(C)$ likewise for the negative ends. 
As in \cite[Lem.\ 5.5(b)]{bn}, we then have have
\begin{equation}
\label{eqn:linkingbound}
\begin{split}
\ell_\tau(C,C') \le &\sum_{i}m_i\cdot \min(\op{wind}_{i,\tau}^+(C),\op{wind}_{i,\tau}^+(C'))\\
& - \sum_{j}n_j \cdot\max(\op{wind}_{j,\tau}^-(C),\op{wind}_{j,\tau}^-(C')).
\end{split}
\end{equation}
Moreover, equality holds if:
\begin{description}
\item{(*)}
For each $i$, the integers $m_i$ and $\min(\op{wind}_{i,\tau}^+(C),\op{wind}_{i,\tau}^+(C'))$ are relatively prime; and for each $j$, the numbers $n_j$ and $\max(\op{wind}_{j,\tau}^-(C),\op{wind}_{j,\tau}^-(C'))$ are relatively prime.
\end{description}

By Lemma~\ref{lem:normalcn}(b), we have
\begin{equation}
\label{eqn:sharpwind}
\begin{split}
w_{i,\tau}^+(C) &= \floor{m_i\theta_{i,\tau}^+},\\
w_{j,\tau}^-(C) &= \ceil{n_j\theta_{j,\tau}^-}.
\end{split}
\end{equation}
The same holds for any $C'\in\M^J_C$. In particular, by the hypothesis (iv), condition (*) above holds, so equality holds in \eqref{eqn:linkingbound}. Putting all of the above together, we obtain
\[
\#(C\cap C') = Q_\tau(C) + \sum_{i}m_i\floor{m_i\theta_{i,\tau}^+} - \sum_{j} n_j\ceil{n_j\theta_{j,\tau}^-}.
\]
This equation implies that $\#(C\cap C')$ does not depend on the choice of $C'\in\M^J_C$.

{\em Step 3.\/} We now show that if $C'\in\M^J_C$ and $C\neq C'$, then $C$ and $C'$ are disjoint in $\R\times Y$.

As in \cite[Prop.\ 3.4, Step 5]{wh}, hypothesis (iii) and condition (*) above imply that if $C'$ is obtained from $C$ by translating a small amount in the $\R$ direction, then $C$ and $C'$ are disjoint. It then follows from Step 2 that $\#(C\cap C')=0$ for all $C'\in\M^J_C$. By intersection positivity, this means that $C$ and $C'$ are disjoint.

{\em Step 4.\/} We now complete the proof.

(a) We know by Step 1 that the projection of $C$ to $Y$ is an immersion. To show that this projection is an embedding, we just need to show that it is injective. (If this map is an injective immersion, then it is also an embedding because the ends of $C$ are asymptotic to Reeb orbits.) If injectivity fails, then there exist $y\in Y$ and distinct $s_1,s_2\in\R$ such that $(s_1,y),(s_2,y)\in C$. Then $C$ intersects the translation of $C$ by $s_2-s_1$. It follows from Step 3 that $C$ equals the translation of $C$ by $s_2-s_1\neq 0$. This leads to all sorts of contradictions. For example, let $(s^{\ast},y^{\ast}) \in C$ be a point such that $y^{\ast}$ does not lie on a Reeb orbit. For large $n$, we would then have that $(n(s_2-s_1)+s^{\ast},y^{\ast}) \in C$, contradicting asymptotic convergence to Reeb orbits. We conclude that the projection of $C$ to $Y$ is an embedding, and the same argument works for any $C'\in\M^J_C$.

(b) If the projections of $C$ and $C'$ to $Y$ are not disjoint, then there exist $y\in Y$ and $s,s'\in\R$ with $(s,y)\in C$ and $(s',y)\in C'$. Thus $C$ intersects the translation of $C'$ by $s-s'$. It follows from Step 3 that $C$ equals the translation of $C'$ by $s-s'$.
\end{proof}

\begin{proof}[Proof of Proposition~\ref{prop:foliation}.]
 (a) We have proved this in Lemma~\ref{lem:embedding}(a).

(b) If $u$ is any immersed $J$-holomorphic curve in $\R\times Y$ with $c_N(u)<\op{ind}(u)$, then $u$ is automatically cut out transversely; see the review in \cite[Lem.\ 4.1]{dc}, and see \cite{wendl-at} for more general automatic transversality results.  In the present case, $c_N(C)=g(C)=h_+(C)=0$, so $\op{ind}(C)=2$, and the above automatic transversality criterion holds for $C$, as well as for every $C'\in\M^J_C$. Thus $\M^J_C/\R$ is a $1$-manifold.

By Lemma~\ref{lem:embedding}(b), the projections to $Y$ of different elements of $\M^J_C/\R$ are disjoint. To complete the proof that these projections give a foliation of an open subset of $Y$, let $C'\in\M^J_C$, let $(s,y)\in C'$, and let $\pi_Y(C')$ denote the projection of $C'$ to $Y$. We need to show that the natural map
\begin{equation}
\label{eqn:foliationchart}
T_{[C']}(\M^J_C/\R) \longrightarrow (N\pi_Y(C'))_y
\end{equation}
is an isomorphism. Here $N\pi_Y(C')$ denotes the normal bundle to $\pi_Y(C')$ in $Y$. By Lemma~\ref{lem:normalcn}(a), the map
\[
T_{C'}\M^J_C \longrightarrow (NC')_{(s,y)}
\]
is injective, hence an isomorphism. It follows from this that the map \eqref{eqn:foliationchart} is an isomorphism.
\end{proof}





